Intelligent Sailing Model for Open Sea Navigation

Autonomous vessels potentially enhance safety and reliability of seaborne trade. To facilitate the development of autonomous vessels, simulations are required to model realistic interactions with other vessels. However, modeling realistic interactive maritime traffic is challenging due to the unstructured environment, coarsely specified traffic rules, and largely varying vessel types. Currently, there is no standard for simulating interactive maritime environments in order to rigorously benchmark autonomous vessel algorithms. In this paper, we introduce the first intelligent sailing model (ISM), which simulates rule-compliant vessels for navigation on the open sea. An ISM vessel reacts to other traffic participants according to maritime traffic rules while at the same time solving a motion planning task characterized by waypoints. In particular, the ISM monitors the applicable rules, generates rule-compliant waypoints accordingly, and utilizes a model predictive control for tracking the waypoints. We evaluate the ISM in two environments: interactive traffic with only ISM vessels and mixed traffic where some vessel trajectories are from recorded real-world maritime traffic data or handcrafted for criticality. Our results show that simulations with many ISM vessels of different vessel types are rule-compliant and scalable. We tested 4,049 critical traffic scenarios. For interactive traffic with ISM vessels, no collisions occurred while goal-reaching rates of about 97 percent were achieved.

==> figures/plotstyle.tex <==
\usepackage{tikz}
\usetikzlibrary{calc}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepgfplotslibrary{fillbetween}
\usepackage[nohyperlinks, nolist]{acronym}
\usepackage{amsmath}
\usepackage{siunitx}
\RequirePackage{times}

\definecolorset{RGB}{PLOT}{}{%
	Brown, 153, 79, 0;%      ok
	Black,   0,   0,   0;%   ok
	Blue, 86, 180, 233;%     ok
	DarkBlue, 0, 101, 189;%  ok
	Orange, 230, 159, 0;%    ok
	DarkOrange, 213, 94, 0;% not ok: (problem with orange)
	Purple, 93, 58, 155;%    ok
	Pink, 220, 38, 127;%     ok
	Red, 227, 27, 35;%       not ok: (problem with DarkOrange)
	Yellow, 255, 195, 37;%   ok
	BluishGreen, 0, 158,  115;%  ok
	ReddishPurple, 204, 121, 167;%  ok
	Olive, 162, 173, 0;%     not ok: (problem with orange)
	Gray, 153, 153, 153;%    not ok: (problem with reddishpurple)
	Cyan, 64, 176, 166;%     not ok: (problem with ReddishPurple)
	DarkPurple, 136, 34, 85 %ok
}

\definecolor{TUMblue}{rgb}{0.00, 0.40, 0.74}
\definecolor{TUMgray}{rgb}{0.85, 0.85, 0.86}
\definecolor{TUMpantone285C}{rgb}{0.00, 0.45, 0.81}
\definecolor{lightblue}{rgb}{0.7529,0.8118,0.9333}
\definecolor{TUMpantone158}{RGB}{227, 114, 34}
\definecolor{TUMpantone383}{RGB}{162, 173, 0}

\pgfplotsset{
	compat=1.16,
	legend image code/.code={ 
		% Set length of legend icon
		\draw[mark repeat=2,mark phase=2]
		plot coordinates {
			(0cm,0cm)
			(0.05cm,0cm)        %% default is (0.3cm,0cm)
			(0.2cm,0cm)         %% default is (0.6cm,0cm)
		};%
	}
}

%\pgfplotsset{compat=1.16} %<-consider using this
\pgfplotsset{hide scale/.style={
		/pgfplots/xtick scale label code/.code={},
		/pgfplots/ytick scale label code/.code={}}}


\providecommand{\filepath}{.}
\newcommand{\figpath}{\filepath/figures/data/}


\newcommand{\accplotwithtwomarkers}[6]{
	\begin{tikzpicture}
		\tikzstyle{every node}=[font=\footnotesize]
		\begin{axis}[hide scale, width=#2,
			height=#3,
			every tick label/.append style={font=\footnotesize},
			label style={font=\footnotesize},
			ymin=-0.3, ymax=0.3,
			xmin=0, xmax=#4,
			xtick distance = 200,
			ytick={-0.3,-0.15,0,0.15,0.3},
			x tick label style={
				/pgf/number format/.cd,
				fixed,
				fixed zerofill,
				precision=0,
				/tikz/.cd
			},
            extra x ticks={#5, #6},
            extra x tick labels={$t_0$, $t_2$},
            extra x tick style={tick label style={yshift=0.35cm, xshift=-0.2cm, font=\tiny}},
			%ylabel={$\mathrm{a}$ in \unit{\meter\per\second\squared}}, %\radian\per\second
			xlabel={Time in \unit{\second}},
			y label style={yshift=-.3em},
			x label style={yshift=.5em},
			legend style={at={(0.99, 0.01)},anchor=south east,font=\normalfont, nodes={scale=0.7, transform shape}},
			legend cell align={left}
			]
			\addplot[mark=none, black, samples=2, domain=0:#4, line width=0.1pt, color=black!40!white, forget plot]{0.0};
			{#1}
   \addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#5,-0.3)(#5,0.3)};
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#6,-0.3)(#6,0.3)};
		\end{axis}
	\end{tikzpicture}
}

\newcommand{\accplotwiththreemarkerszeroonetwo}[7]{
	\begin{tikzpicture}
		\tikzstyle{every node}=[font=\footnotesize]
		\begin{axis}[hide scale, width=#2,
			height=#3,
			every tick label/.append style={font=\footnotesize},
			label style={font=\footnotesize},
			ymin=-0.3, ymax=0.3,
			xmin=0, xmax=#4,
			xtick distance = 200,
			ytick={-0.3,-0.15,0,0.15,0.3},
			x tick label style={
				/pgf/number format/.cd,
				fixed,
				fixed zerofill,
				precision=0,
				/tikz/.cd
			},
            extra x ticks={#5, #6, #7},
            extra x tick labels={$t_0$, $t_1$, $t_2$},
            extra x tick style={tick label style={yshift=0.35cm, xshift=-0.2cm, font=\tiny}},
			ylabel={$\mathrm{a}$ in \unit{\meter\per\second\squared}}, %\radian\per\second
			xlabel={Time in \unit{\second}},
			y label style={yshift=-.3em},
			x label style={yshift=.5em},
			legend style={at={(0.99, 0.01)},anchor=south east,font=\normalfont, nodes={scale=0.7, transform shape}},
			legend cell align={left}
			]
			\addplot[mark=none, black, samples=2, domain=0:#4, line width=0.1pt, color=black!40!white, forget plot]{0.0};
			{#1}
   \addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#5,-0.3)(#5,0.3)};
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#6,-0.3)(#6,0.3)};
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#7,-0.3)(#7,0.3)};
		\end{axis}
	\end{tikzpicture}
}

\newcommand{\accplotwiththreemarkerszerotwothree}[7]{
	\begin{tikzpicture}
		\tikzstyle{every node}=[font=\footnotesize]
		\begin{axis}[hide scale, width=#2,
			height=#3,
			every tick label/.append style={font=\footnotesize},
			label style={font=\footnotesize},
			ymin=-0.3, ymax=0.3,
			xmin=0, xmax=#4,
			xtick distance = 200,
			ytick={-0.3,-0.15,0,0.15,0.3},
			x tick label style={
				/pgf/number format/.cd,
				fixed,
				fixed zerofill,
				precision=0,
				/tikz/.cd
			},
            extra x ticks={#5, #6, #7},
            extra x tick labels={$t_0$, $t_2$, $t_3$},
            extra x tick style={tick label style={yshift=0.35cm, xshift=-0.2cm, font=\tiny}},
			%ylabel={$\mathrm{a}$ in \unit{\meter\per\second\squared}}, %\radian\per\second
			xlabel={Time in \unit{\second}},
			y label style={yshift=-.3em},
			x label style={yshift=.5em},
			legend style={at={(0.99, 0.01)},anchor=south east,font=\normalfont, nodes={scale=0.7, transform shape}},
			legend cell align={left}
			]
			\addplot[mark=none, black, samples=2, domain=0:#4, line width=0.1pt, color=black!40!white, forget plot]{0.0};
			{#1}
   \addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#5,-0.3)(#5,0.3)};
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#6,-0.3)(#6,0.3)};
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#7,-0.3)(#7,0.3)};
		\end{axis}
	\end{tikzpicture}
}


\newcommand{\phiplotwithtwomarkers}[6]{
	\begin{tikzpicture}
		\tikzstyle{every node}=[font=\footnotesize]
		\begin{axis}[hide scale, width=#2,
			height=#3,
			every tick label/.append style={font=\footnotesize},
			label style={font=\footnotesize},
			ymin=-0.05, ymax=0.05,
            %ymin=-0.3, ymax=0.3,
			xmin=0, xmax=#4,
			xtick distance = 200,
			%ytick={-0.3,-0.15,0,0.15,0.3},
            %ytick={-0.1,-0.05,0,0.05,0.1},
            ytick={-0.05,-0.025, 0,0.025,0.05},
			x tick label style={
				/pgf/number format/.cd,
				fixed,
				fixed zerofill,
				precision=0,
				/tikz/.cd
			},
            extra x ticks={#5, #6},
            extra x tick labels={$t_0$, $t_2$},
            extra x tick style={tick label style={yshift=0.35cm, xshift=-0.2cm, font=\tiny}},
			%ylabel={$\mathrm{\omega}$ in \unit{\radian\per\second}}, %
			xlabel={Time in \unit{\second}},
			y label style={yshift=-.3em},
			x label style={yshift=.5em},
			legend style={at={(0.99, 0.01)},anchor=south east,font=\normalfont, nodes={scale=0.7, transform shape}},
			legend cell align={left}
			]
			\addplot[mark=none, black, samples=2, domain=0:#4, line width=0.1pt, color=black!40!white, forget plot]{0.0};
   
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#5,-0.05)(#5,0.05)};
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#6,-0.05)(#6,0.05)};
			{#1}
		\end{axis}
	\end{tikzpicture}
}

\newcommand{\phiplotwiththreemarkerszeroonetwo}[7]{
	\begin{tikzpicture}
		\tikzstyle{every node}=[font=\footnotesize]
		\begin{axis}[hide scale, width=#2,
			height=#3,
			every tick label/.append style={font=\footnotesize},
			label style={font=\footnotesize},
			ymin=-0.05, ymax=0.05,
            %ymin=-0.3, ymax=0.3,
			xmin=0, xmax=#4,
			xtick distance = 200,
			%ytick={-0.3,-0.15,0,0.15,0.3},
            %ytick={-0.1,-0.05,0,0.05,0.1},
            ytick={-0.05,-0.025, 0,0.025,0.05},
			x tick label style={
				/pgf/number format/.cd,
				fixed,
				fixed zerofill,
				precision=0,
				/tikz/.cd
			},
            extra x ticks={#5, #6, #7},
            extra x tick labels={$t_0$, $t_1$, $t_2$},
            extra x tick style={tick label style={yshift=0.35cm, xshift=-0.2cm, font=\tiny}},
			ylabel={$\mathrm{\omega}$ in \unit{\radian\per\second}}, %
			xlabel={Time in \unit{\second}},
			y label style={yshift=-.3em},
			x label style={yshift=.5em},
			legend style={at={(0.99, 0.01)},anchor=south east,font=\normalfont, nodes={scale=0.7, transform shape}},
			legend cell align={left}
			]
			\addplot[mark=none, black, samples=2, domain=0:#4, line width=0.1pt, color=black!40!white, forget plot]{0.0};
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#5,-0.05)(#5,0.05)};
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#6,-0.05)(#6,0.05)};
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#7,-0.05)(#7,0.05)};
			{#1}
		\end{axis}
	\end{tikzpicture}
}

\newcommand{\phiplotwiththreemarkerszerotwothree}[7]{
	\begin{tikzpicture}
		\tikzstyle{every node}=[font=\footnotesize]
		\begin{axis}[hide scale, width=#2,
			height=#3,
			every tick label/.append style={font=\footnotesize},
			label style={font=\footnotesize},
			ymin=-0.05, ymax=0.05,
            %ymin=-0.3, ymax=0.3,
			xmin=0, xmax=#4,
			xtick distance = 200,
			%ytick={-0.3,-0.15,0,0.15,0.3},
            %ytick={-0.1,-0.05,0,0.05,0.1},
            ytick={-0.05,-0.025, 0,0.025,0.05},
			x tick label style={
				/pgf/number format/.cd,
				fixed,
				fixed zerofill,
				precision=0,
				/tikz/.cd
			},
            extra x ticks={#5, #6, #7},
            extra x tick labels={$t_0$, $t_2$, $t_3$},
            extra x tick style={tick label style={yshift=0.35cm, xshift=-0.2cm, font=\tiny}},
			%ylabel={$\mathrm{\omega}$ in \unit{\radian\per\second}}, %
			xlabel={Time in \unit{\second}},
			y label style={yshift=-.3em},
			x label style={yshift=.5em},
			legend style={at={(0.99, 0.01)},anchor=south east,font=\normalfont, nodes={scale=0.7, transform shape}},
			legend cell align={left}
			]
			\addplot[mark=none, black, samples=2, domain=0:#4, line width=0.1pt, color=black!40!white, forget plot]{0.0};
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#5,-0.05)(#5,0.05)};
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#6,-0.05)(#6,0.05)};
\addplot[thick, dashed, samples=50, smooth,domain=0:6,gray] coordinates {(#7,-0.05)(#7,0.05)};
			{#1}
		\end{axis}
	\end{tikzpicture}
}


\newcommand{\trajplot}[8]{ %4-7: ymin ymax xmin xmax 5: yticklabesl
	%\begin{tikzpicture}
		%\tikzstyle{every node}=[font=\footnotesize]
		\begin{axis}[hide scale, width=#2,
			height=#3,
			every tick label/.append style={font=\footnotesize},
			label style={font=\footnotesize},
			ymin=#4, ymax=#5,
			xmin=#6, xmax=#7,
			xtick distance = 300,
			ytick distance = 300,
			x tick label style={
				/pgf/number format/.cd,
				fixed,
				fixed zerofill,
				precision=0,
				/tikz/.cd
			},
            yticklabels={0, 0, 3, 6, 9, 12, 15, 18, 21, 24, 27, 30, 33, 37},
            xticklabels={0, 0, 3, 6, 9, 12, 15, 18, 21, 24, 27, 30},
            xlabel={Position trajectories, axes in $100$ \unit{\meter}},
			x label style={yshift=-.1em},
			legend style={at={(0.99, 0.01)},anchor=south east,font=\normalfont, nodes={scale=0.7, transform shape}},
			legend cell align={left}
			]
			{#1}
		\end{axis}
	%\end{tikzpicture}
}

\newcommand{\trajplotbusy}[8]{ %4-7: ymin ymax xmin xmax 5: yticklabesl
	%\begin{tikzpicture}
		%\tikzstyle{every node}=[font=\footnotesize]
		\begin{axis}[hide scale, width=#2,
			height=#3,
			every tick label/.append style={font=\footnotesize},
			label style={font=\footnotesize},
			ymin=#4, ymax=#5,
			xmin=#6, xmax=#7,
			xtick distance = 300,
			ytick distance = 300,
			x tick label style={
				/pgf/number format/.cd,
				fixed,
				fixed zerofill,
				precision=0,
				/tikz/.cd
			},
            yticklabels={0, 0, 3, 6, 9, 12, 15, 18, 21, 24, 27, 30, 33, 37},
            xticklabels={0, 0, 3, 6, 9, 12, 15, 18, 21, 24, 27, 30},
            xlabel={Position trajectories, axes in $100$ \unit{\meter}},
			x label style={yshift=-.1em},
			legend style={at={(0.99, 0.3)},anchor=south east,font=\normalfont, nodes={scale=0.7, transform shape}},
			legend cell align={left}
			]
			{#1}
		\end{axis}
	%\end{tikzpicture}
}



\newcommand{\plotmeanacc}[2]{
	\addplot [
	mark=None,
	line width=1pt,
	color=#1,
	solid,
	] 
	table[
	x = step,
	y = control_a
	] 
	{\data};
	\addlegendentry{#2}
}


\newcommand{\plotmeanphi}[2]{
	\addplot [
	mark=None,
	line width=1pt,
	color=#1,
	solid,
	] 
	table[
	x = step,
	y = control_omega
	] 
	{\data};
	\addlegendentry{#2}
}


\newcommand{\plottraj}[4]{
	\addplot [
	mark=None,
	line width=1pt,
	color=#1,
	solid,
	] 
	table[
	x = position_x,
	y = position_y
	] 
	{\data};
	\addlegendentry{#2}
}


%% True plots
% --- Figure 3 ---
\newcommand{\plotAccwithtwomarkers}[5]{
    \accplotwithtwomarkers{
		\pgfplotstableread[col sep=comma]{\figpath #1.csv}{\data}
		\plotmeanacc{TUMblue}{Vessel 1}
		\pgfplotstableread[col sep=comma]{\figpath #2.csv}{\data}
		\plotmeanacc{TUMpantone383}{Vessel 2}
		\legend{};
	}{6cm}{3.8cm}{#3}{#4}{#5}
}

\newcommand{\plotAccwiththreemarkerszeroonetwo}[6]{
    \accplotwiththreemarkerszeroonetwo{
		\pgfplotstableread[col sep=comma]{\figpath #1.csv}{\data}
		\plotmeanacc{TUMblue}{Vessel 1}
		\pgfplotstableread[col sep=comma]{\figpath #2.csv}{\data}
		\plotmeanacc{TUMpantone383}{Vessel 2}
		\legend{};
	}{6cm}{3.8cm}{#3}{#4}{#5}{#6}
}

\newcommand{\plotAccwiththreemarkerszerotwothree}[6]{
    \accplotwiththreemarkerszerotwothree{
		\pgfplotstableread[col sep=comma]{\figpath #1.csv}{\data}
		\plotmeanacc{TUMblue}{Vessel 1}
		\pgfplotstableread[col sep=comma]{\figpath #2.csv}{\data}
		\plotmeanacc{TUMpantone383}{Vessel 2} 
		\legend{};
	}{6cm}{3.8cm}{#3}{#4}{#5}{#6}
}


\newcommand{\plotPhiwithtwomarkers}[5]{
    \phiplotwithtwomarkers{
		\pgfplotstableread[col sep=comma]{\figpath #1.csv}{\data}
		\plotmeanphi{TUMblue}{Vessel 1}
		\pgfplotstableread[col sep=comma]{\figpath #2.csv}{\data}
		\plotmeanphi{TUMpantone383}{Vessel 2}
		\legend{};
	}{6cm}{3.8cm}{#3}{#4}{#5}
}

\newcommand{\plotPhiwiththreemarkerszeroonetwo}[6]{
    \phiplotwiththreemarkerszeroonetwo{
		\pgfplotstableread[col sep=comma]{\figpath #1.csv}{\data}
		\plotmeanphi{TUMblue}{Vessel 1}
		\pgfplotstableread[col sep=comma]{\figpath #2.csv}{\data}
		\plotmeanphi{TUMpantone383}{Vessel 2}
		\legend{};
	}{6cm}{3.8cm}{#3}{#4}{#5}{#6}
}

\newcommand{\plotPhiwiththreemarkerszerotwothree}[6]{
    \phiplotwiththreemarkerszerotwothree{
		\pgfplotstableread[col sep=comma]{\figpath #1.csv}{\data}
		\plotmeanphi{TUMblue}{Vessel 1}
		\pgfplotstableread[col sep=comma]{\figpath #2.csv}{\data}
		\plotmeanphi{TUMpantone383}{Vessel 2}
		\legend{};
	}{6cm}{3.8cm}{#3}{#4}{#5}{#6}
}

\newcommand{\plotTrajectoriesGivewayKeep}[9]{ %5-8: ymin ymax xmin xmax ; this will plot in legend first "Giveway" and then "Keep"
	\trajplot{
		{#3}
        \pgfplotstableread[col sep=comma]{\figpath #2.csv}{\data}
		\plottraj{TUMpantone383}{Give-way}{-500}{0}
		\pgfplotstableread[col sep=comma]{\figpath #1.csv}{\data}
		\plottraj{TUMblue}{Stand-on}{-500}{0}
		
		{#4}
	%}{6.93cm}{7.35cm}{#5}{#6}{#7}{#8}{{-1,0,1}}
 	}{6.6cm}{7cm}{#5}{#6}{#7}{#8}{{-1,0,1}} 
}

\newcommand{\plotTrajectoriesGivewayGiveway}[9]{ %5-8: ymin ymax xmin xmax 
	\trajplot{
		{#3}
		
		\pgfplotstableread[col sep=comma]{\figpath #2.csv}{\data}
		\plottraj{TUMpantone383}{Give-way 1}{-500}{0}
       \pgfplotstableread[col sep=comma]{\figpath #1.csv}{\data}
		\plottraj{TUMblue}{Give-way 2}{-500}{0}
		{#4}
	%}{6.93cm}{7.35cm}{#5}{#6}{#7}{#8}{{-1,0,1}}
 	}{6.6cm}{7cm}{#5}{#6}{#7}{#8}{{-1,0,1}} 
}

\newcommand{\plotTrajectoriesKeepGiveway}[9]{ %5-8: ymin ymax xmin xmax 
	\trajplot{
		{#3}
		\pgfplotstableread[col sep=comma]{\figpath #1.csv}{\data}
		\plottraj{TUMblue}{Keep}{-500}{0}
		\pgfplotstableread[col sep=comma]{\figpath #2.csv}{\data}
		\plottraj{TUMpantone383}{Giveway}{-500}{0}
		{#4}
	%}{6.93cm}{7.35cm}{#5}{#6}{#7}{#8}{{-1,0,1}}
 	}{6.6cm}{7cm}{#5}{#6}{#7}{#8}{{-1,0,1}} 
}

\newcommand{\plotTrajectoriesthin}[9]{ %5-8: ymin ymax xmin xmax
	\trajplot{
		{#3}
		\pgfplotstableread[col sep=comma]{\figpath #1.csv}{\data}
		\plottraj{TUMblue}{Vessel 1}{-500}{0}
		\pgfplotstableread[col sep=comma]{\figpath #2.csv}{\data}
		\plottraj{TUMpantone383}{Vessel 2}{-500}{0}
		{#4}
	}{6.2cm}{7cm}{#5}{#6}{#7}{#8}{{-1,0,1}} 
%}{6.51cm}{7.35cm}{#5}{#6}{#7}{#8}{{-1,0,1}}  
}

\newcommand{\plotTrajectoriesverythin}[9]{ %5-8: ymin ymax xmin xmax
	\trajplot{
		{#3}
		\pgfplotstableread[col sep=comma]{\figpath #1.csv}{\data}
		\plottraj{TUMblue}{Vessel 1}{-500}{0}
		\pgfplotstableread[col sep=comma]{\figpath #2.csv}{\data}
		\plottraj{TUMpantone383}{Vessel 2}{-500}{0}
		{#4}
	%}{5.2cm}{7cm}{#5}{#6}{#7}{#8}{{-1,0,1}} 
 }{5.46cm}{7.35cm}{#5}{#6}{#7}{#8}{{-1,0,1}}
 
 %{#8} %{4cm}{7cm}
}


\newcommand{\plotTrajectoriesBusy}[9]{ %5-8: ymin ymax xmin xmax
	\trajplotbusy{
		{#3}
		\pgfplotstableread[col sep=comma]{\figpath busy_ID1001.csv}{\data}
		\plottraj{TUMblue}{Vessel 1}{-500}{0}

		\pgfplotstableread[col sep=comma]{\figpath busy_ID2001.csv}{\data}
		\plottraj{TUMpantone383}{Vessel 2}{-500}{0}

  		\pgfplotstableread[col sep=comma]{\figpath busy_ID3001.csv}{\data}
		\plottraj{PLOTPurple}{Vessel 3}{-500}{0}

  		\pgfplotstableread[col sep=comma]{\figpath busy_ID4001.csv}{\data}
		\plottraj{PLOTDarkOrange}{Vessel 4}{-500}{0}

  		\pgfplotstableread[col sep=comma]{\figpath busy_ID5001.csv}{\data}
		\plottraj{PLOTBluishGreen}{Vessel 5}{-500}{0}

  		\pgfplotstableread[col sep=comma]{\figpath busy_ID6001.csv}{\data}
		\plottraj{PLOTYellow}{Vessel 6}{-500}{0}
  
		{#4}
        %\legend{};
	%}{6.93cm}{7.35cm}{#5}{#6}{#7}{#8}{{-1,0,1}}
 	}{7cm}{7cm}{#5}{#6}{#7}{#8}{{-1,0,1}} 
}






